Analyzing Multiagent Interactions in Traffic Scenes via Topological Braids

We focus on the problem of analyzing multiagent interactions in traffic domains. Understanding the space of behavior of real-world traffic may offer significant advantages for algorithmic design, data-driven methodologies, and benchmarking. However, the high dimensionality of the space and the stochasticity of human behavior may hinder the identification of important interaction patterns. Our key insight is that traffic environments feature significant geometric and temporal structure, leading to highly organized collective behaviors, often drawn from a small set of dominant modes. In this work, we propose a representation based on the formalism of topological braids that can summarize arbitrarily complex multiagent behavior into a compact object of dual geometric and symbolic nature, capturing critical events of interaction. This representation allows us to formally enumerate the space of outcomes in a traffic scene and characterize their complexity. We illustrate the value of the proposed representation in summarizing critical aspects of real-world traffic behavior through a case study on recent driving datasets. We show that despite the density of real-world traffic, observed behavior tends to follow highly organized patterns of low interaction. Our framework may be a valuable tool for evaluating the richness of driving datasets, but also for synthetically designing balanced training datasets or benchmarks.

==> sections/application.tex <==
\section{Case Study: Uncontrolled Intersections}\label{sec:application}

To illustrate the value of the representation of topological braids for driving domains, we consider an application involving navigation at an uncontrolled intersection, i.e., an intersection with no traffic signs or signals.

% \begin{equation}
% \begin{split}
% & \dot{\mathrm{x}}_{i} = u^{i}_{s}\cos(\theta_{i})\\
% & \dot{\mathrm{y}}_{i} = u^{i}_{s}\sin(\theta_{i})\\
% & \dot{\uptheta}_{i} = \frac{u^{i}_{s}}{L}\tan(u_{\phi}^{i})
% \end{split}
% \mbox{,}
% \end{equation}
% Describing the state of agent $i$ as $x_{i}=(\mathrm{x}_{i},\mathrm{y}_{i},\theta_{i})\in SE(2)$, the system kinematics may be written as:

\begin{figure}
\centering
\includegraphics[width = .97\linewidth]{figures/notation.png}
\caption{Illustration of the notation. Having started from state $s_{1}$ and followed a trajectory $\xi_{1}$, the ego car (shown in red), currently in configuration $q_{1}$ and executing a control input $u_{1}$ follows a path $\tau_{1}$ towards its destination $d_{1}$. The figure also lists all quantities about other cars that are observable by the ego car. \label{fig:notation}}
\end{figure}

% \begin{figure*}
% \centering
% \begin{subfigure}{0.23\linewidth}
% \centering
% \includegraphics[trim = {.5cm 0cm 0.2cm 0.1cm}, clip, width = \linewidth]{figures/allpaths.png}
% \caption{The red agent is uncertain of the intended paths of other agents. This uncertainty complicates its decision making.\label{fig:allpaths}}
% \end{subfigure}
% ~
% \begin{subfigure}{0.23\linewidth}
% \centering
% \includegraphics[trim = {0cm 0cm 0.2cm 0.1cm}, clip, width = \linewidth]{figures/controldiagrams.png}
% \caption{Agents' control profiles so far (depicted as graphs with time) are indicative of their intentions. \label{fig:controldiagrams}}
% \end{subfigure}
% ~
% \begin{subfigure}{0.23\linewidth}
% \centering
% \includegraphics[trim = {.9cm 0cm 0.6cm 0cm}, clip, width = \linewidth]{figures/pathsfollowed.png}
% \caption{Top view of the trajectories that agents followed from the beginning to the end of the intersection. \label{fig:pathsfollowed}}
% \end{subfigure}
% ~
% \begin{subfigure}{0.23\linewidth}
% \centering
% \includegraphics[width = \linewidth]{figures/spatiotemporal.png}
% \caption{Projection of agents' trajectories onto the $x$-$t$ plane and topological characterization of emerging trajectory crossings. \label{fig:spatiotemporal}}
% \end{subfigure}
% \caption{The ego agent (red car) enters an unsignalized intersection. Despite unaware of others' destinations (\subref{fig:allpaths}), by observing the joint state history (\subref{fig:controldiagrams}), the ego agent may infer the intentions of others. Based on the inferred intentions, the ego agent may further infer the upcoming sequence of intersection crossings (\subref{fig:pathsfollowed}). The trajectory crossings unveiled in the 2-dimensional projection of \figref{fig:spatiotemporal} reveal crucial properties of the collision-avoidance protocol followed by agents. The formalism of topological braids \citep{artin} allows us to describe the execution of the complete execution of (\subref{fig:pathsfollowed}) as a word composed of symbols (Fig. (\subref{fig:spatiotemporal})) representing pairwise topological relationships among agents' trajectories.\label{fig:introfigs}}
% \end{figure*}

\subsection{Setup}

Consider the 4-way symmetric intersection of \figref{fig:notation} where $n>1$ agents are navigating between different sides. We assume that agent $i$ tracks a legally defined path $\tau_{i}$ (on the right side of the road) connecting a start $s_{i}$ to a destination $d_{i}$. Path $\tau_{i}$ is unknown to any other agent $j\neq i$. Each lane at the intersection is $50m$ long and $3.6m$ wide, whereas each car is represented as a rectangle with a length of $4.7m$ and a width of $1.7m$. 


%We assume that any side $a$ is connected to any different side $b\neq a$ with a unique, publicly known legal path $\tau_{ab}$, lying along the middle of the lane (see \figref{fig:pathsets}). We assume that any agent $i\in \pazocal{N}$ that attempts to reach side $b$ from side $a$ will attempt to track this path, $\tau_{ab}$. 

%All agents track their paths with the same tracking controller $\kappa:V_{i}\to\pazocal{U}_{i}$, taking as input a desired linear velocity $v_{i}\in V_{i}$ in Cartesian coordinates and outputting a control command $u_{i}\in\pazocal{U}_{i}$. This controller is designed based on a feedback linearization technique \citep{Yun92onfeedback} although any other path tracking controller such as e.g., PID or pure pursuit \citep{Coulter-1992-13338} could be used. 

%The main decision variable of our scheme is the speed with which an agent tracks its path; given that speed, the tracking controller outputs a control input $u_{i}\in\pazocal{U}_{i}$ which is directly executed. 






%Thus, for any execution, the set of system paths that could be followed by agents, $\pazocal{T}$, has cardinality $|\pazocal{T}|=3^4=81$. 




%In the following sections, we show that negotiation with just 1-dimensional control inputs in such scenarios can be sufficient for collision-free and efficient navigation.




% \begin{figure}
%     \centering
%     \includegraphics[width = \linewidth]{figures/pathsets.png}
%     \caption{Experimental Setup. Agents' path sets and reference frames are drawn in the same color. Each agent selects a path from its path set (left, right, or forward) and represents braids by assuming a projection plane defined by $x_{i}$ and time (out of the page).}
%     \label{fig:pathsets}
% \end{figure}








%assume that all agents are running a Pure Pursuit Controller \citep{Coulter92} that provides a steering angle $u^{i}_{\phi}$ at the current time step based on a desired path in $\mathrm{x}$-$\mathrm{y}$ coordinates defined by the function $c^{i}(\rho^{i}) \in \mathbb{R}^2$, where $\rho^{i} \in \mathbb{R}$ is a path coordinate.  To calculate the steering angle, the controller uses a lookahead distance parameter $d_l$, defined as the distance ahead of the path position corresponding to the closest point on $c^{i}$ to the agent along the direction of travel.

% Problem \#1 considers point robots (state $x_{i}\in\mathbb{R}^2$) with a 1-dimensional control space $\pazocal{U}\subset\mathbb{R}$, and assumes that all agents follow predefined paths that are publicly known to everyone. The decision-making task in this problem lies in determining a sequence of speeds, i.e., a proper time parametrization of an agent's path that allows for efficient, collision-free motion.

% Problem \#2 also considers point robots with a 1-dimensional control space. In this case, we assume that agents do not have access to the specific paths of others. They do however have access to a universally defined set of paths from which all agents are drawing. These paths connect all possible pairs of sides with each other in a unique way that follows the rules of traffic (using the right lane of the road). In this problem, agents need to incorporate a mechanism for inferring the intended paths of others in their decision-making process.

% Problem \#3 considers point robots with a 2-dimensional control space. In this case, it is assumed that all agents have access to the goals of others but they have no information on how they intend to reach them. Thus, in this case, agents need to incorporate a mechanism for inferring the intended destinations of others in order to make informed decisions about their own actions towards avoiding collisions and reaching their destinations efficiently. 

% Problem \#4 also considers point robots with a 2-dimensional control space. In this case it is assumed that agents have no access to either the paths or the destinations of others. Thus, they should employ a strategy that is robust to this uncertainty.

% Problem \#5 considers volume robots (state $x_{i}\in SE(2)$ contains position and orientation) without holonomic constraints, i.e., agents may execute velocities towards any direction in $SE(2)$. We also assume that agents have access to each other's destinations. The decision-making task for an agent in this problem lies in determining a sequence of 3-dimensional control inputs towards reaching the intended final configuration while avoiding collisions with others. Agents may use the knowledge of others' destinations to their advantage.

% Problem \#6 is exactly the same as problem \#5 but in this case agents do not have access to the destinations of others and they need to follow a robust strategy to avoid collisions.

% \begin{table}[h!]
%   \begin{center}
%     \caption{Description of Considered Planning Problems}
%     \label{tab:tableofproblems}
%     \resizebox{.5\textwidth}{!}{
%     \begin{tabular}{c|l|c|l}
%       Problem & $x_{i}$ & Paths & $u_{i}$\\
%       \hline
%       1 & $\mathbb{R}^2$ & Known & $\mathbb{R}$\\
%       2 & $\mathbb{R}^2$ & Partially known (set) & $\mathbb{R}$\\
%       3 & $\mathbb{R}^2$ & Partially known (goals) & $\mathbb{R}^2$\\
%       \hline       
%       4 & $\mathbb{R}^2$ & Unknown & $\mathbb{R}^2$\\     
%       5 & $SE(2)$ & Partially known (goals) & $SE(2)$\\
%       6 & $SE(2)$ & Unknown & $SE(2)$\\  
%     \end{tabular}
%     }
%   \end{center}
% \end{table}



\begin{figure}
\centering
\includegraphics[width = \linewidth]{figures/inference.png}
\caption{Illustration of the inference architecture at a four-agent intersection crossing scenario. At time $t$, the ego agent (red color), heading to destination $\tau_{1}$, having access to the joint state history $\Xi$, updates its belief about the topology $\beta$ of the emerging multiagent interaction based on beliefs over other agents' new speeds $u_{i}$ and destinations $\tau_{i}$, $i\in\{2,3,4\}$.\label{fig:inference}}
\end{figure}

 

\subsection{Inference over Braids}

%Naively reasoning about the space of multiagent trajectories misses the prevalent effect that structure plays in this domain. The geometric constraints induced by the road structure but also the risk-aversion of agents effectively compress the space of possible outcomes. We formalize this domain insight through the representation of topological braids. For reference, in a 4-agent scenario, the space of braids that could be practically possible for any $n$-agent scenario could be upper-bounded to $S_{b} \leq [2(n-1)]^{D}+1$ under the assumption of a maximum depth $D$ representing the maximum number of generators appearing in a braid word describing the execution. For a 4-agent scenario with $D = 5$ (the depth appearing the most across our 4-agent experiments), this number would be $S_{b} = 7,777$. Note that in practice, the size of the space of relevant topological outcomes may even be significantly smaller than $S_{b}$ depending on the problem setup and agents' state history.

%to make a more coarse prediction focusing on the joint behavior of agents,



%We consider path tracking to be split in two parts: (a) the \textit{negotiation} part, which corresponds to the initial straight-path part of the intersection (denoted as $\pazocal{Q}_{i}^{neg}$ for agent $i$), within which the agent attempts to reach a consensus with others wrt a joint strategy of collision avoidance; (b) the \textit{execution} part, which corresponds to the rest of the path (denoted as $\pazocal{Q}_{i}^{exec}$ for agent $i$), within which the agent tracks the remainder of its path, by maintaining a constant speed. This decision emphasizes the importance of proactive negotiation during the first portion, and provides a natural metric of quality --the count of collisions during the execution part. 


At time $t\in [0,t_{\infty}]$, agent $i$, having access to the complete system state history so far, $\Xi$, maintains a belief $bel_{i}(\beta_{i})=P(\beta_{i}|\Xi)$ over the braid $\beta_{i}\in B_{n}$ that describes the topology of the emerging (future) system trajectory $\Xi' = \Xi_{t\to \infty}$. This braid is extracted upon assuming a projection onto a plane defined by a vector $\hat{\eta}_{i}$ and time $\hat{t}$. For instance, in \figref{fig:braidisarepresentative}, the red agent (agent 1) has set $\hat{\eta}_{1}=\hat{x}$, assuming the projection plane $\hat{x}$-$\hat{t}$.

The braid $\beta_{i}$ is heavily dependent on agents' intended system path $T$. To capture this dependency, we marginalize over $\pazocal{T}_{i}\subseteq\pazocal{T}$, the subset of all system paths for which agent $i$ (the ego agent) follows its intended path:

\begin{equation}
bel_{i}= P(\beta_{i}|\Xi) = \sum_{T\in\pazocal{T}_{i}}P(\beta_{i}|\Xi,T)P(T|\Xi)\mbox{.}\label{eq:bel}
\end{equation}

For a given system path $T$, different braids could possibly emerge, depending on the path tracking behavior of agents. To capture this dependency, we marginalize the probability $P(\beta_{i}|\Xi,T)$ over the set of possible control profiles that could be taken by agents at the current time step:
\begin{equation}
P(\beta_{i}|\Xi,T)=\sum_{U\in\mathbfcal{U}}P(\beta_{i}|\Xi,U,T)P(U|\Xi,T)\mbox{.}\label{eq:bel2}
\end{equation}
Substituting to eq. \eqref{eq:bel}, we get:
\begin{equation}
bel_{i} = \sum_{\pazocal{T}_{i}} \Bigg\{\sum_{\mathbfcal{U}}P(\beta_{i}|\Xi,U,T)P(U|\Xi,T)\Bigg\}P(T|\Xi)\mbox{.}
\label{eq:finalbelief}
\end{equation}
The outlined mechanism combines a local action selection model $P(U|\Xi,T)$ with a model of intent inference $P(T|\Xi)$ and a global behavior prediction model $P(\beta_{i}|\Xi,U,T)$.

\begin{figure}
\centering
\includegraphics[width = .97\linewidth]{figures/flowchart.png}
\caption{Illustration of the decision-making scheme. At every cycle, the ego agent forward simulates a set of distinct futures, classifies them into topological outcomes, and selects the action that minimizes the uncertainty over such outcomes.\label{fig:flowchart}}
\end{figure}

The intention of agent $j\neq i$ over a path $\tau_{j}$ is conditionally independent of the intention of any other agent, given the past system trajectory $\Xi$. The probability over the path intention of agent $j$ does not depend on the trajectories of others. Thus, we simplify the computation of the system path prediction as:
\begin{equation}
P(T|\Xi) = \prod_{j\in \pazocal{N} \backslash i}P(\tau_{j}|\xi_{j})\mbox{,}
\end{equation}
where the product only considers the probabilities over the paths of others, since agent $i$ is certain about its own path.


Similarly, since agents select a control input independently, without having access to the policies of others, we decompose the computation of the control profile prediction as:
\begin{equation}
P(U|\Xi,T) = \prod_{i=1}^{n}P(u_{i}|\Xi,T)\mbox{,}\label{eq:transitionmodel}
\end{equation}
where the distribution $P(u_{i}|\Xi,T)$ represents the control input that agent $i$ executes to make progress along its path $\tau_{i}$, incorporating considerations such as preferred navigation velocity and a local controller class.


The model of inference of eq.~\eqref{eq:finalbelief} focuses on topology prediction, without considerations of collision avoidance. To filter out unsafe braids, we redefine eq. \eqref{eq:finalbelief} by incorporating a model of collision prediction. Define by $c$ a boolean random variable representing the event that $\Xi'$, the emerging future trajectory contains collisions (\texttt{true} for a collision, \texttt{false} for no-collision). Denote by $\tilde{\beta} = (\beta_{i}, \neg c)$ the joint event that $\Xi'$ is both topologically equivalent (ambient-isotopic \citep{murasugi1999study}) to a braid $\beta_{i}\in B_{n}$, \emph{and} not in collision, i.e., $c$ is \texttt{false}. Then the probability that $\tilde{\beta_{i}}$ is true can be computed as:
\begin{equation}
bel_{i}(\tilde{\beta}_{i}) = \sum_{\pazocal{T}} \Bigg\{\sum_{U}P(\tilde{{\beta}}_{i}|\Xi,U,T)P(U|\Xi,T)\Bigg\}P(T|\Xi)\mbox{.}\label{eq:finalfinalbelief}
\end{equation}
The occurrence of a collision is conditionally independent of the emerging braid given the state history, the current control profile and the intended system path; thus, we may compute their joint distribution as:
\begin{equation}
\begin{split}
P(\tilde{\beta}_{i}|\Xi,U,T)=&P(\tilde{\beta}_{i},\neg c|\Xi,U,T)\\ =& P(\neg c|\Xi,U,T,\beta_{i})P(\beta_{i}|\Xi,U,T)\\ =& (1-P(c|\Xi,U,T,\beta_{i}))P(\beta_{i}|\Xi,U,T)\label{eq:finalfinal}
\mbox{.}
\end{split}
\end{equation}



\subsection{Planning with Braids}\label{sec:decisionmaking}


An outcome $\tilde{\beta}_{i}$ represents a class of solutions to the problem of multiagent collision avoidance at the intersection with distinct topological properties. Before execution, multiple classes of solutions could be theoretically possible. However, as execution progresses, the distribution over those classes, $P(\tilde{\beta}_{i}|\Xi,U,T)$, from the perspective of the ego agent (agent $i$) is reshaped as a result of agents' decisions. Our approach is based on the insight that by manipulating agents' actions over time we could enable them to reach a state of clear consensus over a solution $\tilde{\beta}_{i}$ more quickly. To this end, we employ a decision-making mechanism that contributes uncertainty-reducing actions over the emerging solution $\tilde{\beta}_{i}$ by directly minimizing the information entropy of the distribution over future braids(eq.~\eqref{eq:finalfinalbelief}). The lower the Entropy is, the lower the uncertainty, and thus the closer agents are to a consensus over a solution $\tilde{\beta}_{i}$. Besides, the use of the information entropy cost reflects the realization that multiple solutions from $B_{n}$ could be valid solutions to the collision avoidance problem at a given instance. The ego agent behavior could still contribute to collision-free navigation even when there is not a unique winner within $B_{n}$. This decision is motivated and in line with recent work in shared autonomy (e.g., \citet{javdanietal18}).

From the perspective of agent $i$, the uncertainty over a solution $\tilde{\beta}_{i}$ is represented as:
\begin{equation}
H(\tilde{\beta}_{i})=-\sum_{B_{n}}P(\tilde{\beta_{i}}|\Xi)\log P(\tilde{\beta_{i}}|\Xi)\mbox{,}
\end{equation}
where $P(\tilde{\beta_{i}}|\Xi)$ is recovered using eq. \eqref{eq:finalfinalbelief}. In order to contribute towards reducing this uncertainty, agent $i$ selects actions (velocities) that minimize the entropy:
\begin{equation}{}
u_{i}=\arg\min_{u_{i}}H(\tilde{\beta}_{i})\mbox{.}\label{eq:planning}
\end{equation}
Notice that eq.~\eqref{eq:planning} contains the tuple $U$ through the marginalization of eq.~\eqref{eq:finalfinalbelief}. Thus, the optimization scheme outputs the control input $u_{i}$ for agent $i$ that reduces $H(\beta_{i})$ the most in expectation.



\subsection{Implementation}

We assume that agent $i$ has no knowledge of the path $\tau_{j}$ of any other agent $j\neq i\in \pazocal{N}$ while $j$ is in the negotiation stage. However, we assume that $\tau_{j}$ becomes immediately obvious when agent $j$ enters the intersection:
\begin{equation}
P(\tau_{j}|\xi_{j}(t)) = P(\tau_{j}|q_{j}) = 
\begin{cases}
1/m & \textnormal{for}\: q_{j}\in Q^{neg}_{j}\\
1 & \textnormal{for}\: q_{j}\in Q^{exec}_{j}\mbox{,}\\
\end{cases}
\end{equation}
where $q_{j} = \xi_{j}(t)$ is agent $j$'s current state, and $m=3$ is the number of paths that agent $j$ selects from.


% In order to predict the path of agent $j$, agent $i\neq j$ looks for a correspondence between the observed behavior of agent $j$ so far, $\xi_{j}$, and the candidate paths from $\pazocal{T}_{i}$ that agent $j$ is legally allowed to follow, i.e., the paths taking $j$ forward, left or right. The closer agent $j$ is to one of those paths, the more likely it is that it is going to continue along it. Thus, we define:
% \begin{equation}
% P(\tau_{j}|\xi_{j}) = \frac{1}{Z_{T}}e^{-d(\tau_{j},\xi_{j})}\mbox{,}
% \end{equation}
% where $d$ is a distance function between the trajectory followed by agent $j$ so far and the path in consideration $\tau_{j}\in\pazocal{T}_{i}$, and $Z_{T}$ is a normalizer over the path set that agent $j$ could follow.


At time $t$, agent $i$ selects a velocity $v_{i}\in V_{i}^{t}$ and passes it to the controller $\kappa$ which converts it to an executable control command $u_{i}$. The set $V_{i}^{t}$ contains two linear Cartesian velocities pointing towards the next waypoint in $\tau_{i}$: one of low magnitude $|v^{t}_{low}|$ and one of high magnitude $|v_{high}^{t}|$. These magnitudes are fixed throughout the execution and are generally distinct for each agent. We further assume that all agents prefer the higher speed, and that in the beginning of the execution, they start with the high speed. We express this preference in the probability $P(u_{j}|\xi_{j},\tau_{j})$. In the following simulations we assume that agents prefer the high speed with higher probability over the low speed. For each agent, this probability is sampled uniformly from the range $[0.6,0.8]$ and remains fixed throughout the execution. We also assume that each agent assumes that others have the same exact preferences over speeds, i.e., they do \emph{not} know the true preferences of others. This decision introduces a level of uncertainty into an agent's model of behavior for other agents.

% The speed of each agent $u^{i}_{s}$ is calculated based on a desired speed $s_{des}$ and whether collision with other agents is imminent.  Assuming two agents are of length $\ell$, and each are aware of the other's current speed, position and future path, we compute a simple collision avoidance law under the assumption of constant speeds.  Specifically,
% \begin{equation}
%   u^i_{s} = \left\{
%   \begin{array}{lr}
%     s^j\frac{\Delta\rho^{ij} - \frac{\ell}{2}}{\Delta\rho^{ji} + \frac{\ell}{2}}
%     & \textrm{if } s^j\frac{\Delta\rho^{ij} - \frac{\ell}{2}}{\Delta\rho^{ji} + \frac{\ell}{2}}
%     \leq s_{des} \leq
%     s^j\frac{\Delta\rho^{ij} + \frac{\ell}{2}}{\Delta\rho^{ji} - \frac{\ell}{2}} \\
%     s_{des} & \textrm{otherwise}
%   \end{array}
%   \right.
% \end{equation}
% where $\Delta\rho^{ij}$ is the distance from the current path position $\rho^i$ to the intersection point for the paths of agents $i$ and $j$, and $s^j$ is the current speed of agent $j$.  To prevent two agents becoming deadlocked, only one of a pair of agents on a collision course is randomly chosen to adopt the collision avoidance law.  As a simple model of human behavior, we use a Gaussian disturbance model, affecting both the steering and speed inputs to all agents.


The computation of the braid and collision probabilities is based on the forward simulation of system trajectory rollouts. For each path set $T\in\pazocal{T}_{i}$, agent $i$ considers the set of all control profiles drawn from $\mathbfcal{U}$, containing all combinations of control inputs corresponding to high and low magnitude speeds for all agents. For each pair $(T,U)\in T\times\mathbfcal{U}_{i}$, agent $i$ simulates a system trajectory $\Xi'$ by linearly projecting forward all agents from the current system state $\Xi(t)$ towards $T$ with a constant speed $U$. From each trajectory, it extracts a corresponding braid word $\beta_{i}$ (as described in Sec. \ref{sec:trajectoriesbraids}, using BraidLab \citep{braidlab}), and the minimum inter-agent distance $d_{min}$. By repeating this process for all rollouts, agent $i$ constructs a set $B\subset B_{n}$ comprising the set of possible braids that could be realizable in the remainder of the execution under the stated assumptions about agents' behaviors. Each braid $\beta^{*}\in B$ is then evaluated as:
\begin{equation}
P(\beta_{i} = \beta^*|\Xi,U,T) = 
\left\{
  \begin{array}{ll}
    1  & \mbox{if } \beta_{i}=\beta^* \\
    0 & \mbox{otherwise }
  \end{array}
\right.\mbox{.}
\end{equation}
This model acts as a switch that determines which rollouts should be considered for each braid found at the simulation stage. Finally, we model the probability of a collision $P(c|\Xi,U,T,\beta_{i})$ with the following sigmoid model:
\begin{equation}
P(c|\Xi,U,T,\beta_{i})=\frac{1}{1 + e^{a(d_{min}-\delta)}}\mbox{,}
\end{equation}
where $a$ controls the rate of change of the function and $\delta$ denotes a threshold distance beyond which collision is imminent. According to this model, the smaller $d_{min}$ is, it is exponentially more likely to have a collision.


\begin{figure}
\centering
\begin{subfigure}{0.38\linewidth}
\centering
\includegraphics[trim = {2.3cm .5cm 3.3cm .9cm}, clip, width = \linewidth]{figures/numcollisions12agents11goals.eps}
\caption{Frequency of collisions for S1.\label{fig:numcol2agents}}
\end{subfigure}
~
\begin{subfigure}{0.38\linewidth}
\centering
\includegraphics[trim = {2.6cm .5cm 3.3cm .9cm}, clip, width = \linewidth]{figures/maxtime12agents11goals.eps}
\caption{Maximum time to destination for S1.\label{fig:time2agents}}
\end{subfigure}
\\
\begin{subfigure}{0.38\linewidth}
\centering
\includegraphics[trim = {2.3cm .5cm 3.3cm .9cm}, clip, width = \linewidth]{figures/numcollisions123agents111goals.eps}
\caption{Frequency of collisions for S2.\label{fig:numcol3agents}}
\end{subfigure}
~
\begin{subfigure}{0.38\linewidth}
\centering
\includegraphics[trim = {2.6cm .5cm 3.3cm .9cm}, clip, width = \linewidth]{figures/maxtime123agents111goals.eps}
\caption{Maximum time to destination for S2.\label{fig:time3agents}}
\end{subfigure}
\\
\begin{subfigure}{0.38\linewidth}
\centering
\includegraphics[trim = {2.3cm .5cm 3.3cm .9cm}, clip, width = \linewidth]{figures/numcollisions1234agents1111goals.eps}
\caption{Frequency of collisions for S3.\label{fig:numcol4agents}}
\end{subfigure}
~
\begin{subfigure}{0.38\linewidth}
\centering
\includegraphics[trim = {2.6cm .5cm 3.3cm .9cm}, clip, width = \linewidth]{figures/maxtime1234agents1111goals.eps}
\caption{Maximum time to destination for S3.\label{fig:time4agents}}
\end{subfigure}
\caption{Performance evaluation under homogeneous settings: (\subref{fig:numcol2agents}) and (\subref{fig:time2agents}) depict collision frequency and experiment time for S1 (2 agents), computed over 144 experiments; (\subref{fig:numcol3agents}) and (\subref{fig:time3agents}) depict collision frequency and experiment time for S2 (3 agents), computed over 125 experiments; (\subref{fig:numcol4agents}) and (\subref{fig:time4agents}) depict collision frequency and experiment time for S3 (4 agents), computed over 81 experiments. Bars correspond to conditions; error bars indicate standard deviations (assuming a collision is a Bernoulli event) and 25/75 percentiles in the collision frequency and time charts respectively.\label{fig:eval-homogeneous}}
\end{figure}

\subsection{Evaluation I: Homogeneous Setting}\label{sec:eval-homogeneous}

We define three scenarios, involving 2, 3, and 4 agents respectively. For each scenario, we generate a set of experiments by varying agents' speed preferences. We execute each experiment under 5 conditions, each corresponding to a distinct variation of the proposed algorithm, executed by all agents (homogeneous setting). We then measure performance by looking at the frequency of collisions and the maximum experiment time per scenario and condition.

\textbf{Scenarios}:

\noindent S1: Two agents, starting from the bottom and the right sides of the intersection, are moving straight towards the top and left sides respectively. They both draw speeds from $\pazocal{U}_{s1}$ containing 12 evenly spaced speeds within $[5,10]$ ($m/s$). We generate 144 experiments corresponding to the Cartesian product $\pazocal{U}_{s1}^2$. 

\noindent S2: Three agents, starting from the bottom, right and top are moving straight towards the top, left and bottom sides respectively. They draw speeds from $\pazocal{U}_{s2}$, containing 5 evenly spaced speeds within the range $[5,10]$ ($m/s$). We generate 125 experiments corresponding to $\pazocal{U}_{s2}^3$. 

\noindent S3: Four agents, starting from the bottom, right, top, and left, are moving straight towards the top, left, bottom, and right sides respectively. They draw speeds from $\pazocal{U}_{s3}$, containing 3 evenly spaced speeds within the range $[5,10]$ ($m/s$). We generate 81 experiments corresponding to $\pazocal{U}_{s3}^4$. 

\begin{figure}
\centering
\begin{subfigure}{0.48\linewidth}
\centering
\includegraphics[trim = {3cm .1cm 3.2cm .1cm}, clip, width = \linewidth]{figures/scenario36_4agentsC2.eps}
\caption{Agents are running C2. \label{fig:C2}}
\end{subfigure}
~
\begin{subfigure}{0.48\linewidth}
\centering
\includegraphics[trim = {3cm .1cm 3.2cm .1cm}, clip, width = \linewidth]{figures/scenario36_4agentsC4.eps}
\caption{Agents are running C4.\label{fig:C4}}
\end{subfigure}
\caption{Qualitative comparison: Distance covered per agent over the first $3s$ of execution within a 4-agent experiment. The black line indicates arrival at the intersection. We see that agents running C2 have reached a clear ordering of entry to the intersection, effectively corresponding to a consensus. In contrast, agents running C4 are clustered in pairs corresponding to an unclear ordering of intersection crossings.\label{fig:qualitative}}
\end{figure}

\textbf{Conditions}:

\noindent C1: An adaptation of the proposed scheme of eq.~\eqref{eq:spec} for which $w_{i} = 1$, i.e., agents track their desired paths with their desired speeds, without accounting for avoiding collisions with others. This condition serves as a characterization of the intensity of the multiagent encounters at the intersection for each scenario.

\noindent C2: The complete proposed algorithm.

\noindent C3: A modification of the proposed algorithm that assumes knowledge of the paths that other agents are following, i.e, they replace eq.~\eqref{eq:finalfinalbelief} with
\begin{equation}
bel(\tilde{b}_i) = \sum_{U}P(\tilde{{\beta}}_{i}|\Xi,U,T)P(U|\Xi,T)\mbox{.}
\end{equation}

\noindent C4: A variation of C2 that does not use braids for clustering trajectory sets. Specifically, agents reason about the emerging collision-free system trajectory $\tilde{\Xi}_{i}$ (instead of $\tilde{\beta}_{i}$), replacing eq. \eqref{eq:finalfinalbelief} with
\begin{equation}
bel(\tilde{\Xi}_{i}) = P(\tilde{\Xi}_{i}|\Xi,U,T)P(U|\Xi,T)P(T|\Xi)\mbox{.}\label{eq:c4}
\end{equation}

\noindent C5: A modification of C4 that assumes knowledge of the paths that others are following, i.e, C5 replaces eq. \eqref{eq:c4} with
\begin{equation}
bel(\tilde{\Xi}_{i}) = P(\tilde{\Xi}_{i}|\Xi,U,T)P(U|\Xi,T)\mbox{.}\label{eq:c5}
\end{equation}


\textbf{Analysis}:

\noindent Figure \figref{fig:eval-homogeneous} illustrates the performance of the selected algorithms across the three scenarios considered. As expected, C1 results in the highest collision frequency but lowest time to destination for all scenarios (red bars), serving as a characterization of the intensity of the selected scenarios. Our algorithm (C2) achieves consistently low collision frequencies for all scenarios (blue bars). Compared to C4, C2 reduces collision frequency by: 95\% across S1 (\figref{fig:numcol2agents}); 65\% across S2 (\figref{fig:numcol3agents}); 66\% across S3 (\figref{fig:numcol2agents}). C4, leveraging the knowledge of other agents' paths, consistently exhibits lower collision frequency than C5 across all scenarios. The price that C2, and C3 pay is the increased maximum time to destination; it can however be observed that for the more complex scenarios (S2, S3), the time difference is not significant (\figref{fig:time3agents}, \figref{fig:time4agents}). Note that a direct comparison of values across scenarios is not well defined as their parameter spaces (speed combinations) have different dimensionalities. We observe however that the general trends transfer across scenarios.

%Interestingly, we observe that the baselines that do not make use of topological reasoning (C4, C5) exhibit significantly higher collision frequencies but also relatively high times to destination (purple, and yellow bars respectively).

%The outlined findings illustrate the benefits of our approach. We observe that clustering topologically equivalent system trajectories (C2, C3) enables significantly safer navigation than the non-topological baselines (C4, C5) with comparable efficiency, and we point out that this trend scales with the number of agents, across a variety of different experiments. We also observe that knowledge of other agents' destinations provides a gain in safety, which our approach (C1, C2) is able to leverage to a higher extent than the baselines (C4, C5).

We interpret the performance gains as the result of effective incorporation of domain knowledge into decision making. The braid group represents the set of distinct modes that could describe the collective motion of navigating agents. Explicitly reasoning about these modes enables a rational agent to anticipate the effect of its actions on system behavior. Our policy outputs local actions of global outlook that contribute towards reducing uncertainty over the emerging mode. Collectively, this results in implicit coordination, reflected in the reduced collision frequency of C2, C3. To illustrate this point, \figref{fig:qualitative} depicts a comparative qualitative example of the behaviors generated by our policy. For the same experiment from S3 (run in the symmetric intersection of \figref{fig:notation}), we observe that C2 agents (\figref{fig:C2}) quickly converge to a clear order of intersection crossings as a result of their proactive decision making. On the other hand, C4 agents (\figref{fig:C4}), lacking the ability of modeling the complex multiagent dynamics, appear unable to coordinate their crossings and end up colliding. 

\subsection{Evaluation II: Reacting to Inattentive Agents}


Assume that agent 1 is an \emph{inattentive} agent that does \emph{not} account for collision avoidance in its decision making, i.e., navigates by solving eq.~\eqref{eq:spec} for $w_{1}=1$. In this section we investigate the effect of an inattentive agent's behavior to the performance of $n-1$ other rational agents, i.e., agents solving eq.~\ref{eq:spec} with $w_{i}\in (0,1)$, $i \neq 1$. To this end, we redefine the conditions C1-C5 from Sec.~\ref{sec:eval-homogeneous} as C1'-C5' by replacing agent 1 with an inattentive agent (C1' is identical to C1 --we include it as a characterization of the intensity of the scenarios considered). We execute the same scenarios S1-S3 from Sec.~\ref{sec:eval-homogeneous} under conditions C1'-C5'.

\textbf{Analysis}:

\figref{fig:eval-heterogeneous} depicts our findings from running the described scenarios under the new conditions. Overall, we see the majority of the trends from Sec.~\ref{sec:eval-homogeneous} to transfer in this heterogeneous domain. Non-topological methods (C4', C5') tend to perform better in terms of time efficiency than the topological ones (C2', C3'), whereas the latter perform better in terms of collision frequency. The distinction in collision frequency is exemplified as the number of agents (and thus the scenario complexity) increases. While we see that the overall scenario complexity increase results in overall decline in performance across all conditions, C2' and C3' are responding to it better, consistently achieving less than half collisions than C4' and C5' in S2 and S3. This behavior illustrates the ability of our framework to robustly handle less predictable scenarios involving agents that violate the rationality assumption as set by eq.~\eqref{eq:spec}.

The patterns of \figref{fig:eval-heterogeneous} also exhibit a few interesting differences compared to the patterns of \figref{fig:eval-homogeneous}, stemming from the introduction of the inattentive agent. In particular, we see that time efficiency is improved overall --the fact that the inattentive agent leaves the intersection with its preferred high speed results in an emptier workspace faster. We also see that overall C2' and C3' perform comparably, but note a trend of C3' scoring higher than C2' in terms of collision frequency for S1 and S2, despite the fact that it is aware of other agents' destinations. We believe that this might have to do with the fact that C2, considering more topological outcomes is able to react more cautiously to the unpredictable behavior of the inattentive agent.


\begin{figure}
\centering
\begin{subfigure}{0.38\linewidth}
\centering
\includegraphics[trim = {2.3cm .5cm 3.3cm .9cm}, clip, width = \linewidth]{figures/numcollisions12agents11goals-agent1antisocial.eps}
\caption{Frequency of collisions for S1.\label{fig:numcol2agents-agent1antisocial}}
\end{subfigure}
~
\begin{subfigure}{0.38\linewidth}
\centering
\includegraphics[trim = {2.6cm .5cm 3.3cm .9cm}, clip, width = \linewidth]{figures/maxtime12agents11goals-agent1antisocial.eps}
\caption{Maximum time to destination for S1.\label{fig:time2agents-agent1antisocial}}
\end{subfigure}
\\
\begin{subfigure}{0.38\linewidth}
\centering
\includegraphics[trim = {2.3cm .5cm 3.3cm .9cm}, clip, width = \linewidth]{figures/numcollisions123agents111goals-agent1antisocial.eps}
\caption{Frequency of collisions for S2.\label{fig:numcol3agents-agent1antisocial}}
\end{subfigure}
~
\begin{subfigure}{0.38\linewidth}
\centering
\includegraphics[trim = {2.6cm .5cm 3.3cm .9cm}, clip, width = \linewidth]{figures/maxtime123agents111goals-agent1antisocial.eps}
\caption{Maximum time to destination for S2.\label{fig:time3agents-agent1antisocial}}
\end{subfigure}
\\
\begin{subfigure}{0.38\linewidth}
\centering
\includegraphics[trim = {2.3cm .5cm 3.3cm .9cm}, clip, width = \linewidth]{figures/numcollisions1234agents1111goals-agent1antisocial.eps}
\caption{Frequency of collisions for S3.\label{fig:numcol4agents-agent1antisocial}}
\end{subfigure}
~
\begin{subfigure}{0.38\linewidth}
\centering
\includegraphics[trim = {2.6cm .5cm 3.3cm .9cm}, clip, width = \linewidth]{figures/maxtime1234agents1111goals-agent1antisocial.eps}
\caption{Maximum time to destination for S3.\label{fig:time4agents-agent1antisocial}}
\end{subfigure}
\caption{Performance evaluation under heterogeneous settings: (\subref{fig:numcol2agents-agent1antisocial}) and (\subref{fig:time2agents-agent1antisocial}) depict collision frequency and experiment time for S1 (2 agents), computed over 144 experiments; (\subref{fig:numcol3agents-agent1antisocial}) and (\subref{fig:time3agents}) depict collision frequency and experiment time for S2 (3 agents), computed over 125 experiments; (\subref{fig:numcol4agents-agent1antisocial}) and (\subref{fig:time4agents-agent1antisocial}) depict collision frequency and experiment time for S3 (4 agents), computed over 81 experiments. Bars correspond to conditions; error bars indicate standard deviations (assuming collision is a Bernoulli event) and 25/75 percentiles in the collision frequency and time charts respectively.\label{fig:eval-heterogeneous}}
\end{figure}



==> sections/bios.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/mavrogiannis}}]{Christoforos Mavrogiannis}
(S’ 12–M’ 19) received a diploma in mechanical engineering from the National Technical University of Athens, Greece in 2013, and the M.S. and Ph.D. degrees from Cornell University in 2017 and 2019, respectively. 

He is currently a postdoctoral research associate in the Paul G. Allen School of Computer Science \& Engineering at the University of Washington, Seattle. His research interests include multiagent systems, human-robot interaction, and robotic manipulation.


\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/decastro}}]{Jonathan A. DeCastro} (S'12--M'17) received the B.S. and M.S. degrees in mechanical engineering from Virginia Tech in 2001 and 2003, respectively and the M.S. and Ph.D. degrees from Cornell University in 2014 and 2017, respectively. 

He is currently a Research Scientist at the Toyota Research Institute in Cambridge, MA.  His current research interests include formal verification, provable testing strategies, interpretable agent behavior modeling, and applications to robot planning and control.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/srinivasa}}]{Siddhartha S. Srinivasa} (S’02–M’08–SM’16– F’18) received the B.Tech. degree in mechanical engineering from the Indian Institute of Technology Madras, Chennai, India, in 1999 and the Ph.D. degree in robotics from Carnegie Mellon University, Pittsburgh, Pennsylvania, in 2005. He is the Boeing Endowed Professor at the School of Computer Science \& Engineering, University of Washington, Seattle, WA, USA. He works on robotic manipulation, with the goal of enabling robots to perform complex manipulation tasks under uncertainty and clutter, with and around people. To this end, he founded the Personal Robotics Lab in 2005. He is also passionate about building end-to-end systems (HERB, ADA, HRP3, CHIMP, Andy, among others) that integrate perception, planning, and control in the real world. Understanding the interplay between system components has helped produce state-of-the-art algorithms for robotic manipulation, motion planning, object recognition, and pose estimation (MOPED), dense 3-D modeling (CHISEL, now used by Google Project Tango), and mathematical models for human–robot collaboration.
\end{IEEEbiography}

==> sections/planning.tex <==
\section{Planning with Multimodal Inference Enabled by Topological Braids}\label{sec:planning}

In this section, we describe a probabilistic model that links past agents' trajectories to a braid representing the spatiotemporal entanglement of their future trajectories at an intersection domain. \figref{fig:inference} illustrates the setup of the proposed model at a four-agent scenario. Based on this mechanism, we build a decision-making scheme for decentralized motion planning at unsignalized intersections.

\begin{figure}
\centering
\includegraphics[width = \linewidth]{figures/inference.png}
\caption{Illustration of the inference architecture at a four-agent intersection crossing scenario. At time $t$, the ego agent (red color), heading to destination $\tau_{1}$, having access to the joint state history $\Xi$, updates its belief about the topology $\beta$ of the emerging multiagent interaction based on beliefs over other agents' new speeds $u_{i}$ and destinations $\tau_{i}$, $i\in\{2,3,4\}$.\label{fig:inference}}
\end{figure}

\subsection{Multimodal Inference with Topological Braids\label{sec:inference}}

At time $t\in [0,t_{\infty}]$, agent $i$, having access to the complete system state history so far, $\Xi$, maintains a belief $bel_{i}(\beta_{i})=P(\beta_{i}|\Xi)$ over the braid $\beta_{i}\in B_{n}$ that describes the topology of the emerging (future) system trajectory $\Xi' = \Xi_{t\to \infty}$. This braid is extracted upon assuming a projection onto a plane defined by a vector $\hat{\eta}_{i}$ and time $\hat{t}$. For instance, in \figref{fig:braidisarepresentative}, the red agent (agent 1) has set $\hat{\eta}_{1}=\hat{x}$, assuming the projection plane $\hat{x}$-$\hat{t}$.

The braid $\beta_{i}$ is heavily dependent on agents' intended system path $T$. To capture this dependency, we marginalize over $\pazocal{T}_{i}\subseteq\pazocal{T}$, the subset of all system paths for which agent $i$ (the ego agent) follows its intended path:

\begin{equation}
bel_{i}= P(\beta_{i}|\Xi) = \sum_{T\in\pazocal{T}_{i}}P(\beta_{i}|\Xi,T)P(T|\Xi)\mbox{.}\label{eq:bel}
\end{equation}

For a given system path $T$, different braids could possibly emerge, depending on the path tracking behavior of agents. To capture this dependency, we marginalize the probability $P(\beta_{i}|\Xi,T)$ over the set of possible control profiles that could be taken by agents at the current time step:
\begin{equation}
P(\beta_{i}|\Xi,T)=\sum_{U\in\mathbfcal{U}}P(\beta_{i}|\Xi,U,T)P(U|\Xi,T)\mbox{.}\label{eq:bel2}
\end{equation}
Substituting to eq. \eqref{eq:bel}, we get:
\begin{equation}
bel_{i} = \sum_{\pazocal{T}_{i}} \Bigg\{\sum_{\mathbfcal{U}}P(\beta_{i}|\Xi,U,T)P(U|\Xi,T)\Bigg\}P(T|\Xi)\mbox{.}
\label{eq:finalbelief}
\end{equation}
The outlined mechanism combines a local action selection model $P(U|\Xi,T)$ with a model of intent inference $P(T|\Xi)$ and a global behavior prediction model $P(\beta_{i}|\Xi,U,T)$.

\begin{figure}
\centering
\includegraphics[width = .97\linewidth]{figures/flowchart.png}
\caption{Illustration of the decision-making scheme. At every cycle, the ego agent forward simulates a set of distinct futures, classifies them into topological outcomes, and selects the action that minimizes the uncertainty over such outcomes.\label{fig:flowchart}}
\end{figure}

The intention of agent $j\neq i$ over a path $\tau_{j}$ is conditionally independent of the intention of any other agent, given the past system trajectory $\Xi$. The probability over the path intention of agent $j$ does not depend on the trajectories of others. Thus, we simplify the computation of the system path prediction as:
\begin{equation}
P(T|\Xi) = \prod_{j\in \pazocal{N} \backslash i}P(\tau_{j}|\xi_{j})\mbox{,}
\end{equation}
where the product only considers the probabilities over the paths of others, since agent $i$ is certain about its own path.


Similarly, since agents select a control input independently, without having access to the policies of others, we decompose the computation of the control profile prediction as:
\begin{equation}
P(U|\Xi,T) = \prod_{i=1}^{n}P(u_{i}|\Xi,T)\mbox{,}\label{eq:transitionmodel}
\end{equation}
where the distribution $P(u_{i}|\Xi,T)$ represents the control input that agent $i$ executes to make progress along its path $\tau_{i}$, incorporating considerations such as preferred navigation velocity and a local controller class.


The model of inference of eq.~\eqref{eq:finalbelief} focuses on topology prediction, without considerations of collision avoidance. To filter out unsafe braids, we redefine eq. \eqref{eq:finalbelief} by incorporating a model of collision prediction. Define by $c$ a boolean random variable representing the event that $\Xi'$, the emerging future trajectory contains collisions (\texttt{true} for a collision, \texttt{false} for no-collision). Denote by $\tilde{\beta} = (\beta_{i}, \neg c)$ the joint event that $\Xi'$ is both topologically equivalent (ambient-isotopic \citep{murasugi1999study}) to a braid $\beta_{i}\in B_{n}$, \emph{and} not in collision, i.e., $c$ is \texttt{false}. Then the probability that $\tilde{\beta_{i}}$ is true can be computed as:
\begin{equation}
bel_{i}(\tilde{\beta}_{i}) = \sum_{\pazocal{T}} \Bigg\{\sum_{U}P(\tilde{{\beta}}_{i}|\Xi,U,T)P(U|\Xi,T)\Bigg\}P(T|\Xi)\mbox{.}\label{eq:finalfinalbelief}
\end{equation}
The occurrence of a collision is conditionally independent of the emerging braid given the state history, the current control profile and the intended system path; thus, we may compute their joint distribution as:
\begin{equation}
\begin{split}
P(\tilde{\beta}_{i}|\Xi,U,T)=&P(\tilde{\beta}_{i},\neg c|\Xi,U,T)\\ =& P(\neg c|\Xi,U,T,\beta_{i})P(\beta_{i}|\Xi,U,T)\\ =& (1-P(c|\Xi,U,T,\beta_{i}))P(\beta_{i}|\Xi,U,T)\label{eq:finalfinal}
\mbox{.}
\end{split}
\end{equation}



\subsection{Decision Making}\label{sec:decisionmaking}


An outcome $\tilde{\beta}_{i}$ represents a class of solutions to the problem of multiagent collision avoidance at the intersection with distinct topological properties. Before execution, multiple classes of solutions could be theoretically possible. However, as execution progresses, the distribution over those classes, $P(\tilde{\beta}_{i}|\Xi,U,T)$, from the perspective of the ego agent (agent $i$) is reshaped as a result of agents' decisions. Our approach is based on the insight that by manipulating agents' actions over time we could enable them to reach a state of clear consensus over a solution $\tilde{\beta}_{i}$ more quickly. To this end, we employ a decision-making mechanism that contributes uncertainty-reducing actions over the emerging solution $\tilde{\beta}_{i}$ by directly minimizing the information entropy of the distribution over future braids(eq.~\eqref{eq:finalfinalbelief}). The lower the Entropy is, the lower the uncertainty, and thus the closer agents are to a consensus over a solution $\tilde{\beta}_{i}$. Besides, the use of the information entropy cost reflects the realization that multiple solutions from $B_{n}$ could be valid solutions to the collision avoidance problem at a given instance. The ego agent behavior could still contribute to collision-free navigation even when there is not a unique winner within $B_{n}$. This decision is motivated and in line with recent work in shared autonomy (e.g., \citet{javdanietal18}).

From the perspective of agent $i$, the uncertainty over a solution $\tilde{\beta}_{i}$ is represented as:
\begin{equation}
H(\tilde{\beta}_{i})=-\sum_{B_{n}}P(\tilde{\beta_{i}}|\Xi)\log P(\tilde{\beta_{i}}|\Xi)\mbox{,}
\end{equation}
where $P(\tilde{\beta_{i}}|\Xi)$ is recovered using eq. \eqref{eq:finalfinalbelief}. In order to contribute towards reducing this uncertainty, agent $i$ selects actions (velocities) that minimize the entropy:
\begin{equation}{}
u_{i}=\arg\min_{u_{i}}H(\tilde{\beta}_{i})\mbox{.}\label{eq:planning}
\end{equation}
Notice that eq.~\eqref{eq:planning} contains the tuple $U$ through the marginalization of eq.~\eqref{eq:finalfinalbelief}. Thus, the optimization scheme outputs the control input $u_{i}$ for agent $i$ that reduces $H(\beta_{i})$ the most in expectation.


%It should be noted that our goal in this work is to study the convergence to multiagent consensus through the use of topological features in a general-purpose framework. It is possible to extend the framework by considering alternative control policies (e.g., Model Predictive Control (MPC) \citep{Garcia89}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ALGORITHM COMMENTED OUT
% \begin{algorithm}
%   \caption{Min$\char`_$Braid$\char`_$Uncertainty($ \Xi, d, \pazocal{T}, \mathbfcal{U},\epsilon$)}\label{alg:planner}
% \begin{algorithmic}[1]
% \Require $\Xi$ $-$ system state history; $d$ $-$ agent's intended destination; $\pazocal{T}$ $-$ Set of possible path sets; $\delta$ $-$ distance-to-goal threshold.
% \State $AtGoal\gets False$
% \While{$\neg AtGoal$}
% \State $P(T|\Xi)\gets\texttt{Get\char`_Path\char`_Distr}(\pazocal{T},\Xi)$
% \State $B\gets\emptyset$
% \For{$i = 1,\dots, N_{T}$}
% \State $T_{i}\gets \pazocal{T}[i]$
% \State $P(U|\Xi, T)\gets \texttt{Get\char`_Action\char`_Distribution}(\Xi, T_{i}, \mathbfcal{U})$
% \For{$j=1,\dots, N_{U}$}
% \State $U_{j}\gets \mathbfcal{U}[j]$
% \State $\Xi'\gets \texttt{Forward\char`_Simulate}(\Xi, U_{j}, T_{i})$
% \State $ID \gets \texttt{get\char`_Braid\char`_ID}(\Xi')$
% \If{$ID == NULL$}
% \State $B \gets B \cup \beta$
% \State $ID \gets |B|$
% \State $P_{\tilde{\beta}}[ID]\gets 0$
% \EndIf
% \State $P_{c}\gets \texttt{Get\char`_Collision\char`_Prob}(\Xi^{sim})$
% \State $P_{\tilde{\beta}}[ID]\gets P_{\tilde{\beta}}[ID] + \left(1-P_{c}\right)P_{\mathbfcal{U}}[j]P_{\pazocal{T}}[i]$
% \EndFor
% \EndFor
% \State $a\gets \texttt{Minimize\char`_Entropy}(P_{\tilde{B}})$
% \State $x\gets \texttt{Execute\char`_Action}(\Xi, a)$
% \If{$||x-d||<\delta$}
% \State $AtGoal\gets True$
% \EndIf
% \EndWhile
% \State \textbf{return} None%\Comment{The gcd is b}
% %\EndProcedure
% \end{algorithmic}
% \end{algorithm}

% Alg.~\ref{alg:planner} describes our online algorithm that makes use of the outlined decision-making mechanism for planning under uncertainty in multiagent unsignalized intersections. The algorithm runs in replanning cycles until the planning agent is close enough to its destination (closer than $\epsilon$-distance). At every planning cycle, Alg.~\ref{alg:planner} iterates over the path-set and control-profile spaces to update the probability distribution over safe braids and select an action that contributes safe progress towards the agent's destination. In particular, for every path set -- control profile pair $(T,U)$, it performs a forward simulation along a path set $T$, assuming an initial control profile $U$ and a sequence of sampled control profiles until agents reach their destinations. This results in a future trajectory $\Xi^{sim}$, which forms a braid $\beta$. This braid might or might not have been seen before in this planning cycle. Depending on that, the algorithm either stores the new braid in the set $B$ and computes the collision free probability for that braid, $P_{\tilde{B}}[k]$, or updates it by adding the new partial sum to it. Upon iterating over all $(T,U)$ pairs, the algorithm determines and executes an action that minimizes the entropy over the belief distribution over braids. \figref{fig:flowchart} depicts a block diagram illustrating the outlined decision-making process.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ALGORITHM COMMENTED OUT



==> sections/problem-statement.tex <==
\section{Problem Statement}\label{sec:statement}





%where $\pazocal{U}_{i}\subseteq\mathbb{R}\times\mathbb{S}$ is a space of controls


%Agent $i$ starts from an initial state $s_{i}\in \pazocal{Q}$, lying on a side of the intersection, and moves towards a final --unknown to others-- state $d_{i}\in\pazocal{Q}$ lying on a different side. 

%$\dot{q}_{i} = \phi(q_{i}, u_{i})$

%standard car kinematics \citep{Lav06}. Agent $i$ does so by tracking

%, for which it holds that $\tau_{i}(0) = s_{i}$ and $\tau_{i}(1) = d_{i}$, where $I=[0,1]$ is a path parametrization

%, satisfying a specification:
% \begin{equation}
%     u_{i} = \arg\min_{u_{i}\in\pazocal{U}_{i}} w_{i} C_{d}(u_{i}) + (1-w_{i})C_{c}(u_{i})\mbox{,}\label{eq:spec}
% \end{equation} 
% where $\pazocal{U}_{i}\subseteq\mathbb{R}\times\mathbb{S}$ is a space of controls, $C_{d}:\pazocal{U}_{i}\to\mathbb{R}_{\geq 0}$ represents the distance cost-to-go and $C_{c}:\pazocal{U}_{i}\to\mathbb{R}_{\geq 0}$ the collision cost of taking an action in consideration $u_{i}$, and $w_{i} \in (0, 1)$ is a weight --unknown to other agents-- describing agent $i$'s personal compromise over the two costs. Agent $i$ is not aware of the intended path $\tau_{j}$, the destination $d_{j}$ or the exact policy $\pi_{j}$ of agent $j\neq i\in \pazocal{N}$ but assumes that any agent $j\neq i\in \pazocal{N}$ is rational, in the sense that they also optimize for some compromise $w_{j}$ between $C_{d}$ and $C_{c}$. 

%We assume that during execution, agent $i$ has access to the complete system state $Q = (q_{1},\dots, q_{n})\in\pazocal{Q}^n$. Our goal is to design decentralized policies $\pi_{i}$ that enable agents to coordinate safe intersection crossings while following time-efficient trajectories under uncertainty.

